Dynamic Collaborative Path Planning for Remote Assistance of Highly-Automated Vehicles

Given its increasing popularity in recent years, teleoperation technology is now recognized as a robust fallback solution for Automated Driving (AD). Remote Assistance (RA) represents an event-driven class of teleoperation with a distinct division of tasks between the Autonomous Vehicle (AV) and the remote human operator. This paper presents a novel approach for RA of AVs in urban environments. The concept draws inspiration from the potential synergy between highly-automated systems and human operators to collaboratively solve complex driving situations. Utilizing a hybrid algorithm that makes use of the Operational Design Domain (ODD) modification idea, it considers actions that go beyond the nominal operational space. Combined with the advanced cognitive reasoning of the human remote operator, the concept offers features that hold the potential to significantly improve both RA and AD user experiences.

==> tables/2_pipeline.tex <==
\begin{table}[!t]
	\vspace*{-5mm}
	\caption{Approach data inputs and outputs}
	\label{tab:pipeline}
	\centering
	\begin{tblr}{
			stretch=1.25,
			colspec={|Q[l,3.5cm]|Q[l,3.5cm]|},
			rowspec={Q[m]}}
		\hline[1pt]
		\textbf{Input}  & \textbf{Output} \\
		\hline[1pt]
		{
		\tabitem Camera streams\\
		\tabitem Vehicle data \\
		\tabitem HD-Map data\\
		\tabitem Localization data\\
		\tabitem Occupancy grid } & {
		\tabitem Path\\
		\tabitem Modified ODD space}\\
		\hline[1pt]
	\end{tblr}
\end{table}

%{\tabitem HD-Map\\
%	\tabitem Occupancy grid\\
%	\tabitem Camera streams\\
%	\tabitem Localization Data \\}


